Automated Fuzzing of Automotive Control Units

Modern vehicles are governed by a network of Electronic Control Units (ECUs), which are programmed to sense inputs from the driver and the environment, to process these inputs, and to control actuators that, e.g., regulate the engine or even control the steering system. ECUs within a vehicle communicate via automotive bus systems such as the Controller Area Network (CAN), and beyond the vehicles boundaries through upcoming vehicle-to-vehicle and vehicle-to-infrastructure channels. Approaches to manipulate the communication between ECUs for the purpose of security testing and reverse-engineering of vehicular functions have been presented in the past, all of which struggle with automating the detection of system change in response to message injection. In this paper we present our findings with fuzzing CAN networks, in particular while observing individual ECUs with a sensor harness. The harness detects physical responses, which we then use in a oracle functions to inform the fuzzing process. We systematically define fuzzers, fuzzing configurations and oracle functions for testing ECUs. We evaluate our approach based on case studies of commercial instrument clusters and with an experimental framework for CAN authentication. Our results show that the approach is capable of identifying interesting ECU states with a high level of automation. Our approach is applicable in distributed cyber-physical systems beyond automotive computing.

==> Makefile <==

TEXFILES = index.tex acronyms.tex \
           00-abstract.tex 01-intro.tex 02-background.tex \
           03-fuzzing.tex 04-sensors.tex 05-evaluation.tex \
           08-related.tex 10-conclusions.tex

ISPELLPAT= -ktexskip1 +cref,Cref,url

all: index.pdf

spelling: ${TEXFILES}
	for file in ${TEXFILES}; do \
          ispell -t ${ISPELLPAT} -b -d british -p ./index.dict $$file; \
          done
	touch spelling

index.pdf: spelling ${TEXFILES} bibliography.bib
	${MAKE} -C graphics
	latexmk -pdf index.tex
	@echo --- TODOs ------------------------------------------------------
	@grep "todo" ${TEXFILES} ; true
	@grep "TODO" ${TEXFILES} ; true

20191020-siot-werquin.tar: index.pdf
	rm -rf 20191020-siot-werquin
	mkdir 20191020-siot-werquin
	cp *.tex *.bib *.bst *.cls index.dict Makefile \
          20191020-siot-werquin
	cp -r graphics 20191020-siot-werquin
#	${MAKE} -C 20191020-siot-werquin
	cp index.bbl 20191020-siot-werquin/
	tar -cvf 20191020-siot-werquin.tar 20191020-siot-werquin

clean:
	${MAKE} -C graphics clean
	rm -f spelling
	rm -f *.log *.aux *.tex.bak *.fdb_latexmk *.fls
	rm -f *.bbl *.blg

distclean: clean
	rm -f index.pdf



==> graphics/Makefile <==
SVG_FILES       = $(shell ls -- *.svg)
SVG_GRAPHICS    = $(SVG_FILES:.svg=.pdf)
R_FILES         = $(shell ls -- *.r)
R_GRAPHICS      = $(R_FILES:.r=.pdf)
TIKZ_FILES      = $(shell ls -- *.tex)
TIKZ_GRAPHICS   = $(TIKZ_FILES:.tex=.pdf)
GRAPHICS        = $(SVG_GRAPHICS) $(R_GRAPHICS) $(TIKZ_GRAPHICS)

all: ${GRAPHICS}

%.pdf: %.svg
	inkscape --export-pdf=$@ $< \
          --export-text-to-path \
          --export-background="#000000"
%.pdf: %.r
	Rscript $<

%.pdf: %.tex
	pdflatex $<
	pdfcrop $@ $@

clean:
	rm -f *.aux *.bbl *.bbl *.blg *.ent *.fdb_latexmk *.fls *.log *.out

distclean: clean
	rm -f ${GRAPHICS}

